Rethinking Video-Text Understanding: Retrieval from Counterfactually Augmented Data

Recent video-text foundation models have demonstrated strong performance on a wide variety of downstream video understanding tasks. Can these video-text models genuinely understand the contents of natural videos? Standard video-text evaluations could be misleading as many questions can be inferred merely from the objects and contexts in a single frame or biases inherent in the datasets. In this paper, we aim to better assess the capabilities of current video-text models and understand their limitations. We propose a novel evaluation task for video-text understanding, namely retrieval from counterfactually augmented data (RCAD), and a new Feint6K dataset. To succeed on our new evaluation task, models must derive a comprehensive understanding of the video from cross-frame reasoning. Analyses show that previous video-text foundation models can be easily fooled by counterfactually augmented data and are far behind human-level performance. In order to narrow the gap between video-text models and human performance on RCAD, we identify a key limitation of current contrastive approaches on video-text data and introduce LLM-teacher, a more effective approach to learn action semantics by leveraging knowledge obtained from a pretrained large language model. Experiments and analyses show that our approach successfully learn more discriminative action embeddings and improves results on Feint6K when applied to multiple video-text models. Our Feint6K dataset and project page is available at https://feint6k.github.io.

==> tables/main_results.bak.tex <==
\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{clccccccccccccc}
        \toprule
        \multirow{2.5}{*}{{Setting}} & \multirow{2.5}{*}{{Model}} & & \multicolumn{1}{c}{MSR-VTT} & \textcolor{white}{i} & \multicolumn{3}{c}{\OursData (MSR-VTT)} & \textcolor{white}{i} & \multicolumn{1}{c}{VATEX} & \textcolor{white}{i} & \multicolumn{3}{c}{\OursData (VATEX)} \\
        \cmidrule{4-4} \cmidrule{6-8} \cmidrule{10-10} \cmidrule{12-14}
         & & & R@1 & & R@1 & R@2 & MeanR & & R@1 & & R@1 & R@2 & MeanR \\
        \midrule
        & Human & & & & 95.2 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & & & & & 96.8 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & \\
        & Random & & <1e-3 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 16.7 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & & & <1e-3 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 16.7 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & \\
        \midrule \midrule
        \multirow{2.5}{*}{{Zero-Shot}} & CLIP \cite{radford2021learning} & & 26.3 {\scriptsize\textcolor{white}{$\downarrow$1.1}} \\
        & SimVTP \cite{ma2022simvtp} \\
        & InternVideo \cite{wang2022internvideo} & & 37.5 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 45.8 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 63.6 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 2.3 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 76.9 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 44.1 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 63.9 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 2.3 {\scriptsize\textcolor{white}{$\downarrow$1.1}} \\
        \midrule \midrule
        \multirow{2.5}{*}{{Finetuned}} & CLIP4Clip \cite{luo2022clip4clip} \\
        & SimVTP \cite{ma2022simvtp} \\
        & \emph{\ \ w /} \OursMethod \& binary \\
        & \emph{\ \ w /} \OursMethod \& logits \\
        & InternVideo \cite{wang2022internvideo} & & 49.1 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 58.6 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 80.2 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 1.8 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 87.9 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & & 58.2 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 76.9 {\scriptsize\textcolor{white}{$\downarrow$1.1}} & 1.9 {\scriptsize\textcolor{white}{$\downarrow$1.1}} \\
        & \emph{\ \ w /} \OursMethod \& binary & & 48.2 {\scriptsize\textcolor{ablation_red}{$\downarrow$0.9}} & & 64.2 {\scriptsize\textcolor{ablation_green}{$\uparrow$5.6}} & 82.5 {\scriptsize\textcolor{ablation_green}{$\uparrow$2.3}} & 1.7 {\scriptsize\textcolor{ablation_green}{$\downarrow$0.1}} & & 85.2 {\scriptsize\textcolor{ablation_red}{$\downarrow$2.7}} & & 63.8 {\scriptsize\textcolor{ablation_green}{$\uparrow$5.6}} & 80.5 {\scriptsize\textcolor{ablation_green}{$\uparrow$3.6}} & 1.7 {\scriptsize\textcolor{ablation_green}{$\downarrow$0.2}} \\
        & \emph{\ \ w /} \OursMethod \& logits & & 48.9 {\scriptsize\textcolor{ablation_red}{$\downarrow$0.2}} & & 65.7 {\scriptsize\textcolor{ablation_green}{$\uparrow$7.1}} & 83.8 {\scriptsize\textcolor{ablation_green}{$\uparrow$3.6}} & 1.7 {\scriptsize\textcolor{ablation_green}{$\downarrow$0.1}} & & 87.3 {\scriptsize\textcolor{ablation_red}{$\downarrow$0.6}} & & 65.6 {\scriptsize\textcolor{ablation_green}{$\uparrow$7.4}} & 81.7 {\scriptsize\textcolor{ablation_green}{$\uparrow$4.8}} & 1.7 {\scriptsize\textcolor{ablation_green}{$\downarrow$0.2}} \\
        \bottomrule
    \end{tabular}}
    \vspace{.1in}
    \caption{Performance of standard video-to-text retrieval on MSR-VTT dataset \cite{xu2016msr} and VATEX dataset \cite{wang2019vatex}, as compared to performance of retrieval from counterfactually-augmented data on our \OursData dataset. In the ``zero-shot'' setting, models are evaluated after the pretraining stage, while in the ``finetuned'' setting, models are finetuned on the training set of MSR-VTT or VATEX.}
    \label{tab:main_results}
\end{table}

